Synergy: Resource Sensitive DNN Scheduling in Multi-Tenant Clusters

Training Deep Neural Networks (DNNs) is a widely popular workload in both enterprises and cloud data centers. Existing schedulers for DNN training consider GPU as the dominant resource, and allocate other resources such as CPU and memory proportional to the number of GPUs requested by the job. Unfortunately, these schedulers do not consider the impact of a job's sensitivity to allocation of CPU, memory, and storage resources. In this work, we propose Synergy, a resource-sensitive scheduler for shared GPU clusters. Synergy infers the sensitivity of DNNs to different resources using optimistic profiling; some jobs might benefit from more than the GPU-proportional allocation and some jobs might not be affected by less than GPU-proportional allocation. Synergy performs such multi-resource workload-aware assignments across a set of jobs scheduled on shared multi-tenant clusters using a new near-optimal online algorithm. Our experiments show that workload-aware CPU and memory allocations can improve average JCT up to 3.4x when compared to traditional GPU-proportional scheduling.

==> ack.tex <==
\section*{Acknowledgements}

We thank our shepherd Ravi Netravali, the anonymous OSDI reviewers,  members of the UT SaSLab, and many of our MSR colleagues for their invaluable feedback that made this work better. Sincere thanks to the fellow Project Fiddle interns Kshiteej Mahajan and Andrew Or for their contributions to the simulator infrastructure. We thank Microsoft Research for their generous support of JM’s internships, and for the many resources required to develop and evaluate this work.
%This work was done during an internship at Microsoft Research as part of Project Fiddle. 
%We sincerely thank MSR Labs for their generous support in procuring the many resources required for this work. 
%This work was supported by NSF CAREER \#1751277 and donations from VMware, Google, and Facebook.

==> background.tex <==
\section{Background}
In this section, we briefly describe DNN scheduling and introduce the terminology used in the rest of the paper.

\vheading{Scheduling DNN training jobs}. Training a DNN is a resource intensive and long-running task (order of hours to days). In enterprise, production, or large reserach clusters, DNN training is carried out in a shared, multi-tenant cluster where users submit their job scripts, specifying the number of GPUs required to train. A scheduler (YARN~\cite{}, or DNN specific ones~\cite{}) maps this job to the available GPU resources in the cluster. 

\vheading{\fair allocation}
In addition to the GPU (user-given), each DNN job requires CPU to pre-process the dataset, and memory to cache the dataset during training. Existing DNN schedulers in literature~\cite{gandiva, gavel, themis}, and those used in real-world GPU clusters~\cite{philly}, allocate CPU and memory resources to a job using a \fair allocation. For instance, consider a server with 4 GPUs, 12 CPUs and 200 GB memory. The \fair allocation for 1 GPU-job is 3 CPUs and 50GB memory. If a job ia allocated  GPUs on this server, then it is given 6 CPUs and 100GB memory.

\vheading{Scheduling policy and mechanism}
When jobs are submitted to a scheduler, a scheduling policy such as First In, First Out (FIFO), Shortest Remaining Time First (SRTF), or Least Attained Service (LAS) decides the next job ($J$) to be run on the cluster. A scheduling mechanism then identifies where job $J$ should be run, and how much resources to allocate to the job. In this work, we do not propose a new scheduling policy; we propose a scheduling mechanism that appropriately allocates resources, and maps jobs onto available servers.


==> eval.tex <==

\section{Evaluation}

\input{tables/tbl-sku}
\subsection{Experimental setup}
We run experiments on both a physical and simulated cluster.

\vheading{Clusters}. We use two distinct server configurations for our experiments as shown in
Table~\ref{tbl-sku}. Both our servers have 500GB DRAM, 24 physical CPU cores
, and 8 GPUs per server. Both these server types are a part of internal
clusters at a large cloud provider; they resemble publicly available information on
typical production cluster SKUs~\cite{philly,jeon2019analysis}.
In all our experiments, fair-share CPU allocation is 3 cores per GPU and fair-share
memory allocation is 62.5GB per GPU.

\vheading{Models}. Our experiments consider 14 different DNNs (CNNs, RNNs, and LSTMs) across a variety of tasks such as image classification (AlexNet, ResNet18, ShuffleNet, SqueezeNet, MobileNet, ResNet50, VGG11), speech recognition (DeepSpeech), music classification (M5), language translation (GNMT), and language modeling (BERT-Large, BERT-base, Transformer-XL). All experiments are performed on PyTorch 1.1.0 using the state-of-the-art NVIDIA data loading pipeline, DALI. 

\vheading{Traces}. Talk about traces for real and simulated experiments


\vheading{Policies and metrics}. We show evaluation for 4 different polices; FIFO, SRTF, LAS, and FTF.

\subsection{Microbenchmarks}
\label{sec-example}
We now show how workload-aware scheduling can improve average JCT on a \confssd server using two examples for a FIFO scheduling 
policy. 

\input{fig-dali/fig-example}
\vheading{Example 1 : CPU sensitivity}. Consider two job requests; a ResNet18 job requesting 4 GPUs and training for 2 epochs on the 550GB OpenImages dataset, and a GNMT job requesting 4 GPUs and training for 2 epochs on the 16GB WMT dataset. The state-of-the-art schedulers that provision GPU as the dominant resource will co-locate these jobs on a server (has 8 GPUs in total) and allocate 12 CPUs and 250GB memory to each job ( fair-share). \scheduler on the other hand, will co-locate these jobs on the same server, but allocates 23 CPUs and 450GB memory to Resnet18 and 1CPU and 50GB memory to GNMT. As shown in Figure~\ref{fig-example}a, \scheduler's decisions does not impact the training time of GNMT, but results in a 2\myx improvement in the training time of ResNet18, reducing both makespan and average JCT.

\vheading{Example 2 : Memory sensitivity}.

\vheading{Example 3 : Local Storage sensitivity}. Consider two job requests; a ResNet18 job requesting 4 GPUs and training for 2 epochs on the 550GB OpenImages dataset, and a M5 job requesting 4 GPUs and training for 2 epochs on the 500GB FMA dataset. The baseline scheduler that is agnostic of the resource sensitivity of DNN jobs will co-locate these jobs on the same physical server. However, \scheduler identifies that both these jobs are storage-bandwidth intensive; if placed on the same server, they will throttle the storage bandwidth and degrade the performance of both jobs. Therefore \scheduler schedules these jobs on different servers and speeds up both jobs significantly as shown in Figure~\ref{fig-example}b.




\subsection{End-to-End Physical Cluster Experiments}
For our physical cluster experiments we run a workload agnostic and workload-aware policy in two different scenarios. Both 
cases use an appropriately sized trace that keeps the cluster fully loaded.
(1) A continuous trace optimizing average JCT using LAS scheduling policy. (2) A static trace optimizing for makespan
using FIFO. The results are shown in Table x

\input{tables/eval-deployment}
\input{fig-dali/fig-eval-deploy}
We compare the observed results from physical experiments to the same trace replayed on our simulator. As shown in Table x, 
the difference between metrics in real and simulated clusters are < y\%, demonstrating the fidelity of the simulator.

\subsection{End-to-end results in simulation}

\vheading{FIFO}. Average JCT for steady-state jobs in te cluster as we vary cluster load for both single-GPU trace and multi-GPU trace is in shown in Fig~\ref{fig-eval-sim-fifo}
\input{fig-dali/fig-sim-1gpu}


\vheading{LAS}.  Average JCT for steady-state jobs in te cluster as we vary cluster load for both single-GPU trace and multi-GPU trace in shown in Fig~\ref{fig-eval-sim-las}
\input{fig-dali/fig-sim-1gpu-las}

\vheading{Comparison to Tetris and DRF}

\subsection{Evaluation of optimistic profiling}
\vheading{Efficacy of profiling}. Compare the profiled vs real throughputs as we vary CPU and memory
for a Res18 job in Fig~\ref{fig-eval-prof-validate}
\input{fig-dali/fig-profiling-validation}

\subsection{Evaluation of SAM}

\vheading{Scalability of optimal algorithm}

\vheading{Resource utilization and fragmentation}. 
\input{fig-dali/fig-sim-gpu-frag}

\vheading{Timeline of a job in \sysname}




==> fig-dali/fig-data-sensitivity.tex <==
 \begin{figure*}[!t]

  \centering 

  \includegraphics[width=0.8\linewidth]{graphs-dali/data-sensitivity.png} 
   
  
    \mycaption{Data sensitivity}{This graph shows total time to train 70 epochs of ResNet50 on a cluster of \confssd for varying number of job migrations. Every migration results in a high one-time overhead to fetch the dataset locally, whereas a data-aware scheduler will eliminate this cost by scheduling storage-sensitive jobs only on servers where the dataset is present locally.}
  %\vspace{-3mm}
  \label{fig-data-sensitivity}

\end{figure*}

==> fig-dali/fig-eval-cpu-util.tex <==
\begin{figure}[!tbh]
	\centering
  \includegraphics[width=.4\textwidth]{graphs-sim/eval-cpu_util.png}
	
 \mycaption{CPU utilization}{This graph plots the cluster CPU utilization at low load. \fair scheduling underutilizes the available CPU resources while \sysname is able to efficiently utilize spare resources to improve cluster metrics.}
\label{fig-eval-cpu-util}
\end{figure}

==> fig-dali/fig-eval-deploy.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=.45\textwidth, height=5cm]{graphs-deploy/cdf_jct_static_fifo.png}
 %\subfloat[Static Trace (FIFO) Trace\label{fig-sim-fifo-single}]{{\includegraphics[width=.45\textwidth, height=5cm]{graphs-deploy/cdf_jct_static_fifo.png} }}%
%\qquad
%\subfloat[Dynamic Trace (SRTF) Trace\label{fig-sim-fifo-multi}]{{\includegraphics[width=.45\textwidth, height=5cm]{graphs-deploy/cdf_jct_static_fifo.png} }}%
	
 \mycaption{\todo{Update for (2)}CDF of job completion time}{This graph compares the baseline \fair mechanism with \systune for a dynamic trace with SRTF.}
\label{fig-eval-deploy}
\end{figure}

==> fig-dali/fig-eval-philly-fifo.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=.4\textwidth]{graphs-sim/philly_fifo_cdf.png} 
	
	\caption{CDF of JCT for FIFO scheduling with Philly trace}
	\label{fig-eval-philly-fifo}
\end{figure}

==> fig-dali/fig-eval-scalability.tex <==
 \begin{figure}[!t]

  \centering 

  \includegraphics[width=0.4\textwidth]{graphs-sim/scalability.png} 
   

    \mycaption{Scalability of the scheduling mechanism}{This graph plots the scheduling overhead per round with \sysopt and \systune. With \sysopt the scheduling overhead increases exponentially with cluster size.}

  \label{fig-eval-scalability}

\end{figure}

==> fig-dali/fig-example.tex <==
 \begin{figure*}[!t]

  \centering 

  \includegraphics[width=1\linewidth]{graphs-dali/example.png} 
   
  
    \mycaption{Example of \scheduler decisions}{This graph the improvement of JCT when scheduled using \scheduler. In (a), \scheduler improves JCT by allocating CPU and memory in a workload-aware manner between the two jobs co-scheduled on the same server. In (b) \scheduler decides to place the two storage-sensitive jobs on different servers, thereby speeding up both jobs.}
  %\vspace{-3mm}
  \label{fig-example}

\end{figure*}

==> fig-dali/fig-mem-sensitivity.tex <==
 \begin{figure}[!t]

  \centering 

  \includegraphics[width=0.95\linewidth]{graphs-dali/mem-sensitivity.png} 
   
  
    \mycaption{Memory sensitivity of DNNs}{This graph shows the training speed for ResNet18 and GNMT for a single-GPU training for varying memory sizes that cache different percentage of input datasets. We see that GNMT is unaffected by memory allocation, while ResNet18 shows significant improvement in performance as we increase memory.}
  %\vspace{-3mm}
  \label{fig-mem-sensitivity}

\end{figure}

==> fig-dali/fig-motivation.tex <==
\begin{figure}[!t]
%\minipage[b]{0.45\textwidth}
  \includegraphics[width=0.45\textwidth]{graphs-dali/cpu-sensitivity-small.png}
  \vspace{-1em}
  \mycaption{CPU allocation sensitivity}{This graph shows the per-epoch training time for different DNNs as we increase their CPU allocation. \fair CPU allocation for this server is 3 CPUs per GPU. We see that some models achieve the same epoch time with fewer than \fair CPU, while others see upto 3\myx speedup by increasing their CPU allocation to above \fair.}
  \label{fig-motivation}
%\endminipage\hfill
%\minipage[b]{0.45\textwidth}
%  \includegraphics[width=\linewidth]{graphs-dali/mem-sensitivity.png}
   %\vspace*{-2.5em}
%  \caption{Memory allocation sensitivity}\label{fig-mem}
%\endminipage\hfill
%\minipage[b]{0.33\textwidth}%
%  \includegraphics[width=\linewidth]{graphs-dali/data-sensitivity.png}
   %\vspace*{-2.5em}
%  \caption{Remote storage sensitivity}\label{fig-data}
%\endminipage
  \vspace*{-1.3em}
\end{figure}

==> fig-dali/fig-sim-1gpu-las.tex <==
\begin{figure*}[!htb]
	\centering
 \subfloat[LAS-Single GPU Trace\label{fig-sim-fifo-single}]{{\includegraphics[width=.45\textwidth, height=5cm]{graphs-sim/single-las-50-0-50.png} }}%
\qquad
\subfloat[LAS-Muti GPU Trace\label{fig-sim-fifo-multi}]{{\includegraphics[width=.45\textwidth, height=5cm]{graphs-sim/multi-las-50-0-50.png} }}%
	
 \mycaption{Average JCT for LAS Scheduling}{The graphs compare the baseline fair-share LAS policy with Synergy-based LAS policies.}
\label{fig-eval-sim-las}
\end{figure*}

==> fig-dali/fig-sim-1gpu.tex <==
\begin{figure*}[!htb]
	\centering
 \subfloat[FIFO-Single GPU Trace\label{fig-sim-fifo-single}]{{\includegraphics[width=.45\textwidth, height=5cm]{graphs-sim/single-fifo-20-70-10.png} }}%
\qquad
\subfloat[FIFO-Muti GPU Trace\label{fig-sim-fifo-multi}]{{\includegraphics[width=.45\textwidth, height=5cm]{graphs-sim/multi-fifo-20-70-10.png} }}%
	
 \mycaption{Average JCT for FIFO Scheduling}{The graphs compare the baseline fai-share fifo policy with Synergy-based FIFO policies.}
\label{fig-eval-sim-fifo}
\end{figure*}

==> fig-dali/fig-sim-fifo.tex <==
\begin{figure*}[!htb]
	\centering
 \subfloat[Avg JCT vs cluster load Trace\label{fig-sim-fifo-jct}]{{\includegraphics[width=.45\textwidth]{graphs-sim/fifo-single-jct-2-7-1.png} }}%
\qquad
\subfloat[CDF of JCT at load = 8 jobs/hr\label{fig-sim-fifo-cdf}]{{\includegraphics[width=.45\textwidth]{graphs-sim/fifo-single-cdf-2-7-1.png} }}%
	
 \mycaption{Average JCT for FIFO Scheduling}{The graphs compare the baseline fai-share fifo policy with Synergy-based FIFO policies.}
\label{fig-eval-sim-fifo}
\end{figure*}

==> fig-dali/fig-sim-las-multi.tex <==
\begin{figure*}[!htb]
	\centering
 \subfloat[Avg JCT vs cluster load Trace\label{fig-sim-las-jct}]{{\includegraphics[width=.45\textwidth]{graphs-sim/las-multi-jct-2-7-1.png} }}%
\qquad
\subfloat[CDF of JCT at load = 5 jobs/hr\label{fig-sim-las-cdf}]{{\includegraphics[width=.45\textwidth]{graphs-sim/las_multi-cdf-2-7-1.png} }}%
	
 \mycaption{Average JCT for FIFO Scheduling}{The graphs compare the baseline fai-share fifo policy with Synergy-based FIFO policies.}
\label{fig-eval-sim-las}
\end{figure*}

==> tables/tbl-analysis-sku.tex <==

\begin{table*}[!t]
  \small
  \centering
  \ra{1.1}
 \begin{tabular}{cccccccc}
	\toprule[1pt]
	     \textbf{\emph{}} & GPU  & GPU  & Storage & Rand Read \\ 
	     \textbf{\emph{}} & Config & Mem(GB) & Media & (MBps)\\ 
	     \midrule
         \texttt{SSD-V100} & 8xV100 & 32 &  SSD & 530 \\
         \texttt{HDD-1080Ti} & 8x1080Ti & 11 & HDD & 15 -- 50 \\
	\bottomrule[1pt]
   \end{tabular}
  \vspace{-1em}
    \mycaption{Server configurations used in this work}{We use two representative ML optimized server SKUs; each server has 24 CPU cores, 500\gb DRAM, and 8 GPUs}
       %\vspace{-2em}
\label{tbl-analysis-sku}
\end{table*}



==> tables/tbl-analysis-summary.tex <==
\newcommand\VRule[1][\arrayrulewidth]{\vrule width #1}
\setlength{\tabcolsep}{3pt}
\begin{table*}[!h]
  \small
  \centering
  \ra{1.2}
 \begin{tabular}{!{\VRule[1pt]}m{0.435\textwidth}!{\VRule[1pt]}m{0.52\textwidth}!{\VRule[1pt]}}
	\specialrule{1.2pt}{0pt}{0pt}
	\rowcolor{grey} \centering
    \textbf{\emph{Finding}} & \Centering\textbf{\emph{\sysname Insights}}\\
    \specialrule{0.8pt}{0pt}{0pt}
    \rowcolor{white}
    OS Page Cache is inefficient for DNN training due to thrashing & Optimize DNN cache to eliminate thrashing across epochs (\textit{\minio} \sref{sec-minio})\\
    \specialrule{0.5pt}{0pt}{0pt}
    Lack of coordination among local caches lead to
    redundant \vio in distributed training across servers & Local caches of servers can be coordinated to fetch data from the remote cache to overcome storage \vio bottlenecks (\textit{Partitioned Cache} \sref{sec-part-cache}) \\
    \specialrule{0.5pt}{0pt}{0pt}
    No coordination in HP search leads to
    redundant \vio \& prep & HP search jobs must coordinate data fetch \& prep (\textit{Coordinated Prep} \sref{sec-coord-prep})\\
%    \specialrule{0.5pt}{0pt}{0pt}
%    DNNs need 3 -- 24 CPU cores per GPU for prep & Hardware must be upgraded carefully and in a balanced manner \\
%    \specialrule{0.5pt}{0pt}{0pt}
%    DNNs spend upto 65\% of epoch time in pre-processing data & We need optimized pre-processing libraries, or better data formats to speed up data augmentation.\\
	\specialrule{1.2pt}{0pt}{0pt}
   \end{tabular}
   \vspace{-0.5em}
    \caption{Key findings and implications of our analysis of data stalls}
    \vspace{-1em}
\label{tbl-analysis-summary}
\end{table*}



==> tables/tbl-dataset-models.tex <==

\begin{table}[!t]
  \small
  \centering
  \ra{1.1}

 \begin{tabular}{l@{\hskip10pt}r@{\hskip15pt}l@{\hskip5pt}r@{\hskip25pt}r@{\hskip10pt}}
	\toprule[1.2pt]
	     Task & Model & & Dataset & Size\\ 
	     \midrule
		\multirow{7}{*}{\shortstack[l]{Image \\Classification}}  & Shufflenetv2~\cite{zhang2018shufflenet} & \rdelim\}{7}{3mm}[] & &\\
		& AlexNet~\cite{krizhevsky2012imagenet} & & ImageNet-22k~\cite{imagenet-22k}  & 1.3TB \\
		& Resnet18~\cite{he2016deep} & & & \\
		& SqueezeNet~\cite{iandola2016squeezenet} & & OpenImages-Extended~\cite{kuznetsova2018open, sarincrowdsource} & 645GB\\
		& MobileNetv2~\cite{sandler2018mobilenetv2} & & & \\ 
		& ResNet50~\cite{he2016deep} & & Imagenet-1k~\cite{russakovsky2015imagenet} & 146GB \\
		& VGG11~\cite{simonyan2014very} & & & \\
	\midrule
	Obj Detection & SSD+Res18~\cite{liu2016ssd} & & OpenImages~\cite{kuznetsova2018open} & 561GB \\
	\midrule
	Audio Classify & M5~\cite{dai2017very} & & Free Music~\cite{defferrard2016fma} & 950GB \\
%	\midrule
%	Language & Bert-Large~\cite{devlin2018bert} & Wikipedia \& \\
%	Modeling & & BookCorpus~\cite{zhu2015aligning}  (110)\\
%	\midrule
%	Translation & GNMT~\cite{wu2016google} & WMT16~\cite{wmt16} (16)\\
	\bottomrule[1.2pt]
   \end{tabular}
   \vspace{-0.5em}
    \mycaption{Models and datasets used in this work}{}
\label{tbl-dataset-models}
   \vspace{0.2em}
\end{table}



==> tables/tbl-dist-mint-net.tex <==

\begin{table}[!t]
  \small
  \centering
  \ra{1.1}
 \begin{tabular}{cccccc}
	\toprule[1pt]
	%Nodes  & 2 & 3 & 4 \\
	& \multicolumn{2}{c}{AlexNet (Mbps)} & \multicolumn{2}{c}{ResNet50 (Mbps)}\\
	Nodes & DALI & \sysname & DALI& \sysname \\
	\midrule
	2 & 0.59 & 13.92 & 1.02 & 5.45 \\
	3 & 0.66 & 14.08 & 1.11 & 5.69 \\
	4 & 0.66 & 15.09 & 1.18 & 5.76 \\
	%DALI (Gbps) & 0.59 & 0.66 & 0.66 \\
	%\sysname (Gbps) & 13.92 & 14.08 & 15.09 \\
	\bottomrule[1pt]
   \end{tabular}
%   \vspace{2pt}
    \mycaption{Network activity during co-ordinated caching}{}
\label{tbl-eval-net}
\end{table}



==> tables/tbl-eval-fetch-miss.tex <==
%\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\setlength\mylength{\dimexpr.5\columnwidth-10\tabcolsep-0.5\arrayrulewidth\relax}
\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
  
   \begin{tabular}{lrrr}
  	\toprule[1pt]
  	 & DALI-seq & DALI-shuffle & \sysname \\
  	\midrule
  
  	\emph{Cache miss}  & 66\% & 53\% & 35\%  \\
  	\emph{Disk IO (GB)} & 422 & 340 & 225\\

  	\bottomrule[1pt]
  \end{tabular}
  
   \vspace{2pt}
   \mycaption{Impact on fetch misses and disk IO}{When training
     ResNet18 on OpenImages (645GB), \sysname reduces cache misses
     from 66\% to 35\%. \confssd caches 65\% of the dataset, so this
     is the minimum miss rate.}
\label{tbl-eval-fetch-miss}
\end{table}



==> tables/tbl-eval-hp-cached-small.tex <==

\begin{table}[!t]
  \small
  \centering
  \ra{1.1}
  
   \begin{tabular}{c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c}
  	\toprule[1pt]
  	%\multicolumn{2}{c}{Models} & ShN & AN & RN18 & SqN & MN & RN50 & V11 \\
  	Models &  ShN & AN & RN18 & SqN & MN & RN50 & V11 \\
  	\midrule
  	%Speed	&   DALI & 1441 & 1399 & 1056 & 835 & 752 & 569 & 552 \\
  	Speed & 1.8\myx & 1.9\myx & 1.5\myx & 1.5\myx & 1.4\myx & 1.2\myx & 1.2\myx \\
  	\bottomrule[1pt]
  \end{tabular}
  
   \vspace{2pt}
    \mycaption{HP search with \sysname on a fully cached dataset}{On \confssd, when training with the small ImageNet-1k dataset that fits in memory, \sysname provides upto 1.9\myx speedup by eliminating redundant pre-processing \small{(ShN-ShuffleNet, AN-AlexNet, RN18-Resnet18, SqN-SqueezeNet, MN-MobileNet, RN50-ResNet50, V11-VGG11)}}
\label{tbl-hp-cached-small}
\end{table}



==> tables/tbl-eval-hp-cached.tex <==
%\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\setlength\mylength{\dimexpr.5\columnwidth-10\tabcolsep-0.5\arrayrulewidth\relax}
\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
  
   \begin{tabular}{lrrr}
  	\toprule[1pt]
  	& \multicolumn{2}{c}{Per job speed (Samples/s)}\\
  	 Model  & DALI & \sysname \\
  	\midrule
  	ShuffleNet & 1441 & 1.81\myx \\
	AlexNet & 1399 & 1.87\myx \\
	ResNet18 & 1056 & 1.53\myx \\
	SqueezeNet & 835 & 1.50\myx \\
	MobileNet & 752 & 1.35\myx \\
	ResNet50 & 569 & 1.21\myx \\
	VGG11 & 552 & 1.22\myx \\
  	\bottomrule[1pt]
  \end{tabular}
  
   \vspace{2pt}
    \mycaption{HP search with \sysname on a fully cached dataset}{On \confssd, when training with the small ImageNet-1k dataset that fits in memory, \sysname provides upto 1.87\myx speedup by eliminating redundant pre-processing}
\label{tbl-hp-cached}
\end{table}



==> tables/tbl-eval-storage-miss.tex <==
%\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newlength\mylengthnew
\setlength\mylengthnew{\dimexpr.5\columnwidth-10\tabcolsep-0.5\arrayrulewidth\relax}
\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
 \begin{tabular}{lrrrrr}
	\toprule[1pt]
         \textbf{\emph{Caching}} & 100\% & 70\% & 55\% & 35\% & 20\%\\
         \midrule
          \textbf{\emph{Page Cache}}  & 0\% & 46\% & 66\% & 84\%  & 97\% \\
           \textbf{\emph{\mint}}  & 0\% & 30\% & 47\% & 65\%  & 81\% \\
	\bottomrule[1pt]
   \end{tabular}
   \vspace{2pt}
    \mycaption{Storage Misses}{Percentage of storage miss in the page cache and \mint caching policy.}
    %(LRU policy) and the \mint caching policy. \mint results in 20\% lower storage misses on average compared to page cache. }
    \vspace{-2em}
\label{tbl-eval-storage-miss}

\end{table}



==> tables/tbl-eval-util.tex <==
\begin{table*}[t!]
\ra{1}
\begin{minipage}[b]{.35\textwidth}
	\centering
	\begin{tabular}{ |c | c | c | c | c | }
		\hline
		Server & GPU & CPU \\ \hline
		Proportional & 100\% & 64\% \\ \hline
		Greedy & 90\% & 85\% \\ \hline
		
		\hline
		\multirow{2}*{$S_2$} & $J3$ & 4 & 12 & 250 \\ \cline{2-5}
		&$J4$ & 4 & 12 & 250 \\ \hline
	\end{tabular} \\
	\captionof{table}{Schedule-Proportional}
	\label{tbl-motivation-ex-sched-1}
\end{minipage}\qquad
\begin{minipage}[b]{.35\textwidth}
	\centering
	\begin{tabular}{ |c | c | c | c | c | }
		\hline
		Server & Job & GPU & CPU & Mem \\ \hline
		\multirow{2}*{$S_1$} & $J1$ & 4 & 23 & 400 \\ \cline{2-5}
		& $J3$ & 4 & 1 & 100 \\ \hline
		\hline
		\multirow{2}*{$S_2$} & $J2$ & 4 & 12 & 450 \\ \cline{2-5}
		&$J4$ & 4 & 12 & 50 \\ \hline
	\end{tabular} \\
	\captionof{table}{Schedule-Resource Sensitive}
	\label{tbl-motivation-ex-sched-2}
\end{minipage}\qquad
\vspace*{-3em}
\end{table*}


==> tables/tbl-philly-simtex.tex <==

\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
 \begin{tabular}{cccc}
	\toprule[1pt]
	      %Policy  & GPU-proportional & \sysname  \\ 
	      %\midrule
	%	FIFO & 73  & 62 \\
	%	SRTF & 11.2 & 8.8 \\
	%	LAS & 9.7 & 8.2\\
	%	FTF & 184 & 159\\
	%Policy & SRTF & FIFO & FTF \\
	%\midrule
	%GPU-prop. & 11.2 & 73 & 184 \\
	%\sysname & 8.8 & 62 & 159 \\
	& \multicolumn{3}{c}{Avg JCT(hrs)}\\
		Policy & SRTF & LAS & FIFO \\
	\midrule
	GPU-prop. & 30 & 32 & 71 \\
	\sysname & 26 & 28 & 62 \\
	
	\bottomrule[1pt]
   \end{tabular}
    \mycaption{Average JCT with \sysname}{This table shows the average JCT on a 512-GPU cluster using production trace with a (20,70,10) split across different scheduling policies}
\label{tbl-philly-eval}
\end{table}



==> tables/tbl-sku.tex <==

\begin{table*}[!t]
  \small
  \centering
  \ra{1.3}
 \begin{tabular}{ccccccc}
	\toprule[1pt]
	      & GPU  & GPU DRAM & CPU  & DRAM  & Storage & Read Thr\\ 
	      & model & (GB) & cores & (GB) & type & (MBps) \\
	      \midrule
         \textbf{\confssd} & 8*V100  & 32 & 24 & 500 & SSD & 530 \\
          \textbf{\confhdd} & 8*1080Ti  & 11 & 24 & 500 & HDD & 15 -- 50 \\
	\bottomrule[1pt]
   \end{tabular}
    \mycaption{Server configurations used in this work}{We use two representative ML server SKUs; both are a part of an internal cluster at a large cloud provider.}
\label{tbl-sku}
\end{table*}



==> tables/tbl-tensorflow-small.tex <==
\setlength\mylength{\dimexpr.5\columnwidth-10\tabcolsep-0.5\arrayrulewidth\relax}
\begin{table}[!t]
    \small
 	\centering
 	\ra{0.9}
 	
 	  \begin{tabular}{@{}c|c|cc@{}}
 		\toprule[1.2pt]
 		%      & \multicolumn{3}{c}{\% dataset cached}\\
 		\% dataset cached  &   8-GPU training & \multicolumn{2}{c}{8-job HP search}\\
 			(Size : 146GB) &  Cache Miss	   &   Disk IO (GB) & Read amp \\
 		\midrule
 		50\% & 91\% & 860 &  6.14\myx \\
 		35\% & 94\% & 1010 & 7.21\myx \\
 		25\% & 97\% &  1019 & 7.28\myx \\
 		\bottomrule[1.2pt]
 	\end{tabular}
 	\vspace{-0.5em}
    \mycaption{Data stalls in Tensorflow}{The fundamental problems that result in data stalls-inefficient caching and thrashing due to lack of coordination in HP search, exist in TensorFlow.}
\label{tbl-analysis-tf-small}
	%\vspace{-1.5em}
\end{table}



==> tables/tbl-tool.tex <==

\begin{table}[!t]
  \small
  \centering
  \ra{1.1}
 \begin{tabular}{cccccc}
	\toprule[1pt] 
	 \% dataset cached $(x)$ & 25\% & 35\% & 50\%  & 100\% \\
	     \midrule
         \emph{$F_{predicted}$} & 6226 & 7164 & 9225 & 9727  \\
         \emph{$F_{empirical}$} & 6130 & 7118 & 9022 & 9484 \\
	\bottomrule[1pt]
   \end{tabular}
%   \vspace{2pt}
    \caption{Training speed (samples/s) predicted by the \tool is atmost
    4\% different from empirical values.}
\label{tbl-tool}
\end{table}


